Stochastic effects of waves on currents in the ocean mixed layer

This paper introduces an energy-preserving stochastic model for studying wave effects on currents in the ocean mixing layer. The model is called stochastic forcing by Lie transport (SFLT). The SFLT model is derived here from a stochastic constrained variational principle, so it has a Kelvin circulation theorem. The examples of SFLT given here treat 3D Euler fluid flow, rotating shallow water dynamics and the Euler-Boussinesq equations. In each example, one sees the effect of stochastic Stokes drift and material entrainment in the generation of fluid circulation. We also present an Eulerian-averaged SFLT model (EA SFLT), based on decomposing the Eulerian solutions of the energy-conserving SFLT model into sums of their expectations and fluctuations.

==> SALT.tex <==
\section{Stochastic advection by Lie transport (SALT)}\label{sec: SDP SALT noise}{app: SALT}

\subsection{Deterministic semidirect-product coadjoint motion for ideal fluids}
\begin{proposition}[Euler-Poincar\'e theorem \cite{HMR1998}]
	The Euler-Poincar\'e (EP) equations of a reduced Lagrangian $\ell(u, a)$, $\ell: \mathfrak{X}\times V^* \rightarrow \mathbb{R}$ defined over the space of smooth vector fields with elements $u\in \mathfrak{X}$ acting by Lie derivative on elements $a\in V^*$ of a vector space $V^*$are written as \cite{HMR1998}
	\begin{align}
	\frac{d}{dt}\frac{\delta \ell}{\delta u} + \ad^*_u \frac{\delta \ell}{\delta u} - \frac{\delta \ell}{\delta a}\diamond a = 0, \quad \frac{d}{dt}a + \mathsterling_u a=0.
	\label{EPeqn}
	\end{align}
\end{proposition}\noindent
In the EP equation in \eqref{EPeqn}, the variational derivative is defined as usual by,
\begin{align}
\delta \ell (u,a) = \frac{d}{d\ep}\bigg|_{\ep=0}\ell (u_\ep,a_\ep)
= \left\langle\,\frac{\delta \ell}{\delta u}\,,\,\delta u\,\right\rangle_{\mathfrak{X}}
+ \left\langle\,\frac{\delta \ell}{\delta a}\,,\,\delta a\,\right\rangle_V\,.
\label{VarDeriv-def}
\end{align}
The quantities $a\in V^*$ and $\delta \ell / \delta a \in V$ in \eqref{VarDeriv-def} are dual to each other under the $L^2$ pairing $\langle\,\cdot\,,\,\cdot\,\rangle_V:V\times V^*\to\mathbb{R}$. Likewise, the velocity vector field $u\in \mathfrak{X}$ and momentum 1-form density $m := \delta \ell / \delta u \in \mathfrak{X}^*$ are dual to each other under  the $L^2$ pairing $\langle\,\cdot\,,\,\cdot\,\rangle_\mathfrak{X}:\mathfrak{X}\times \mathfrak{X}^*\to\mathbb{R}$. In terms of these pairings and the Lie derivative operator $\mathcal{L}_u$ with respect to the vector field $u\in \mathfrak{X}$, the coadjoint operator  $\ad_u^*$ and the diamond operator $(\diamond)$ in \eqref{EPeqn} are defined by 
\begin{align}
\Scp{\ad^*_u \frac{\delta \ell}{\delta u} }{v}_\mathfrak{X} 
:= \Scp{\frac{\delta \ell}{\delta u}}{- \mathcal{L}_u v }_\mathfrak{X}
=: \Scp{\frac{\delta \ell}{\delta u}}{\ad_u v }_\mathfrak{X},
\label{ad-star-def}
\end{align}
where $v\in \mathfrak{X}$, and $\ad:\mathfrak{X}\times\mathfrak{X}\to \mathfrak{X}$ is defined as $\ad_u v := - [u,v] := - (u^jv_{,j}^i-v^ju_{,j}^i)\p_i$, and
\begin{align}
\Scp{b \diamond a}{v}_\mathfrak{X} := \Scp{b}{- \mathcal{L}_v a }_V.
\label{diamond-def}
\end{align}
As we shall see later, the coadjoint operator  $\ad_u^*$ and the diamond operator $(\diamond)$ enter together in \eqref{EPeqn} as a form of coadjoint motion for semidirect product action of the Lie algebra 

\begin{proposition}[The EP equation \eqref{EPeqn} also follows from the HPVP]
The EP equation in \eqref{EPeqn} can be derived by direct calculation from the following Hamilton-Pontryagin variational principle (HPVP)
\begin{align}
0 = \delta S = \delta \int^b_a \Big(\ell(u,a) + \SCP{m}{\dot{g}g^{-1} - u} + \SCP{b}{a_0g^{-1} - a}\Big)\, dt,
\label{HPVP-def}
\end{align}
where $m\in \mathfrak{X}^*$, $b\in V$, $g\in G$ and the variations are taken to be arbitrary. 
\end{proposition}

\subsection{Stochastic semidirect-product coadjoint fluid motion with SALT noise}
To add noise in the SALT form to the deterministic HPVP in \eqref{HPVP-def}, we introduce the following stochastic variational principle, cf. \cite{Holm2015},\footnote{Note: we can choose separate (uncorrelated) Brownian motions in the $m$ and $a$ equations in \eqref{StochHPVP-def} by choosing $h_i(m,a) = h^m_i(m) + h^a_i(a)$ for the Stratonovich noise, $\circ dW^i_t$. The choice of Stratonovich noise enables the standard calculus chain rule and product rule to be used for the operations of differentiation and integration by parts, in which variational principles are defined.}
\begin{align}
0=\delta S = \delta \int^b_a \Big(\ell(u,a)\,dt + \SCP{m}{\rmd g\, g^{-1} - u\,dt} + \SCP{ \rmd b}{a_0g^{-1} - a} - \sum_i h_i(m,a)\circ dW^i_t\Big)\,.
\label{StochHPVP-def}
\end{align}
For brevity of notation, we will suppress the subscript labels in the pairings whenever the meaning is clear.  The symbol $\rmd$ in \eqref{StochHPVP-def} abbreviates stochastic time integrations. The action integral $S$ in \eqref{StochHPVP-def} is defined in the framework of variational principles with semimartingale constraints which was established in \cite{SC2020}. As we shall see below, the semimartingale nature of a Lagrange multiplier which imposes one of these semimartingale constraints emerges in the context of the full system of equations, which is obtained after the variations have been taken.   
The Hamiltonian functions $h_i(m,a)$ on $\mathfrak{X}^*\times V^*$  in \eqref{StochHPVP-def} will be prescribed here without discussing how they would be obtained in practice, e.g., via data assimilation. The data assimilation procedure for SALT is discussed, e.g., in \cite{CCHOS18a,CCHOS18}. 

\paragraph{Euler-Poincar\'e (EP) Lagrangian formulation.}
Taking arbitrary variations in the stochastic HPVP in equation \eqref{StochHPVP-def} yields the following determining  relations among the variables, 
\begin{align*}
0&=\int_a^b \SCP{\frac{\delta \ell}{\delta u}}{\delta u}\,dt + \SCP{\frac{\delta \ell}{\delta a}}{\delta a}\,dt + \SCP{\delta m}{\rmd g\,g^{-1} - u\,dt} + \SCP{ \rmd b}{a_0\delta g^{-1}- \delta a} + \SCP{\delta  \rmd b}{a_0 g^{-1}-a}\\
& \quad- \SCP{\frac{\delta h_i}{\delta m}}{\delta m}\circ dW_t^i - \SCP{\frac{\delta h_i}{\delta a}}{\delta a}\circ dW_t^i + \SCP{m}{\delta(\rmd g\, g^{-1}) - \delta u\,dt}\\
& = \int_a^b \SCP{\frac{\delta \ell}{\delta u}}{\delta u}\,dt + \SCP{\frac{\delta \ell}{\delta a}}{\delta a}\,dt + \SCP{\delta m}{\rmd g\,g^{-1} - u\,dt} + \SCP{ \rmd b}{-a\eta- \delta a} + \SCP{\delta \rmd b}{a_0 g^{-1}-a}\\
& \quad- \SCP{\frac{\delta h_i}{\delta m}}{\delta m}\circ dW_t^i - \SCP{\frac{\delta h_i}{\delta a}}{\delta a}\circ dW_t^i + \SCP{m}{\rmd \eta - \ad_{\rmd g\,g^{-1}}\eta - \delta u\,dt}\,.
\end{align*}
Here, $\eta = \delta g\,g^{-1}$ and natural boundary terms have been assumed. Collecting terms among the variational relations gives the following set of equations, which turn out to involve four semimartingales,
\begin{align}
\begin{split}
&\frac{\delta \ell}{\delta u} = m, \quad \frac{\delta \ell}{\delta a} = b, \quad 
\rmd g\,g^{-1} = u\,dt + \sum_i \frac{\delta h_i}{\delta m}\circ dW^i_t, \quad  \rmd b = \frac{\delta \ell}{\delta a}\,dt - \sum_i \frac{\delta h_i}{\delta a}\circ dW_t^i, \\
&\rmd m = - \ad^*_{\rmd g\,g^{-1}}m +  \rmd b \diamond a, \quad \rmd a = -\mathsterling_{\rmd g\,g^{-1}}a.
\end{split} \label{eq:EP eq parts}
\end{align}
Thus the SALT EP equations are found to be
\begin{align}
\rmd \frac{\delta \ell}{\delta u} = -\, \ad^*_{\rmd g\,g^{-1}}\frac{\delta \ell}{\delta u} + \left(\frac{\delta \ell}{\delta a}\,dt - \sum_i \frac{\delta h_i}{\delta a}\circ dW_t^i\right) \diamond a
\,, \quad 
\rmd a = -\mathsterling_{\rmd g\,g^{-1}} a\,,
\label{eq:StochEPeqns}
\end{align}
where the definition of $\rmd g\,g^{-1}$ are taken from \eqref{eq:EP eq parts}. For a similar, but more rigorous approach to the derivation of these equations, see \cite{SC2020}.

\paragraph{Lie-Poisson (LP) Hamiltonian formulation.}
Using the Legendre transform, $h(m,a) = \SCP{m}{u} - \ell(u,a)$ and taking variations yields
\begin{align}
\frac{\delta \ell}{\delta u} = m\,, \quad \frac{\delta h}{\delta m} = u\,, \quad \frac{\delta h}{\delta a} = -\frac{\delta \ell}{\delta a}\,,
\end{align}
and the corresponding SALT Lie-Poisson (LP) Hamiltonian equations obtained after a Legendre transform are
\begin{align}
\begin{split}
\rmd m = - \ad^*_{\rmd x_t}m - \left(\frac{\delta h}{\delta a}\,dt 
+ \sum_i \frac{\delta h_i}{\delta a}\circ dW_t^i\right) \diamond a
\,, \quad \rmd a = -\mathsterling_{\rmd x_t} a\,,
\end{split} \label{eq:SLP eq SALT}
\end{align}
where the Lagrangian path $\rmd x_t = \rmd g\,g^{-1}$ Legendre-transforms to the Hamiltonian side as
\begin{align}
\rmd x_t = \frac{\delta h}{\delta m}\,dt + \sum_i \frac{\delta h_i}{\delta m}\circ dW^i_t
\,.
\label{LagPath-SALT}
\end{align} 

By using the $\ad^*$ operator for semidirect product Lie algebras defined in appendix \ref{app: semidirect ad^*}, the LP equations \eqref{eq:SLP eq SALT} can be written equivalently in the following compact form,
\begin{align*}
\rmd (m,a) = -\ad^*_{(\rmd x_t,  \rmd b)}(m,a), \quad \text{where }  \rmd b = -\frac{\delta h}{\delta a}\,dt - \sum_i \frac{\delta h_i}{\delta a}\circ dW_t^i.
\end{align*}

\begin{remark}[Stochastic reduced Hamiltonian phase space variational principle for SALT]
	The SALT equations \eqref{eq:SLP eq SALT} can be derived from a stochastic reduced Hamilton phase-space variational principle, namely,
	\begin{align*}
	0=\delta S = \delta \int^b_a \SCP{m}{\rmd g\, g^{-1}} + \SCP{\rmd b}{a_0g^{-1} - a} - h(m, a)\,dt - \sum_i h_i(m,a)\circ dW^i_t,
	\end{align*}
	where the variations $\delta m, \delta g, \delta a$ and $\delta( b)$ are taken to be arbitrary.     
\end{remark}

The SALT Hamiltonian equations in \eqref{eq:SLP eq SALT} can be arranged into the Lie-Poisson (LP)  operator form
\begin{align}
\rmd \begin{bmatrix}m \\ a \end{bmatrix} = -
\begin{bmatrix}
\ad^*_{\fbox{}} m & \fbox{}\diamond a \\
\mathsterling_{\fbox{}}a & 0 
\end{bmatrix}
\begin{bmatrix}
\frac{\delta h}{\delta m}\,dt + \sum_i \frac{\delta h_i}{\delta m} \circ dW^i_t 
\\
\frac{\delta h}{\delta a}\,dt + \sum_i \frac{\delta h_i}{\delta a} \circ dW^i_t 
\end{bmatrix}\,,
\label{eq:SALT-LPB}
\end{align}
The Lie-Poisson operator in \eqref{eq:SALT-LPB} preserves the Casimirs of its deterministic counterpart, since the Poisson structures remains the same. However, the Hamiltonian is now a semimartingale, so energy depends explicitly on time and, hence, is no longer preserved.

\begin{framed}{Referee suggestions: Move to appendix}
\paragraph{Kelvin-Noether theorem.}
The SALT Lie-Poisson (LP) Hamiltonian equations in \eqref{eq:SLP eq SALT} also possess a Kelvin-Noether theorem. 
To understand this statement, consider the following $G$-equivariant map
$\mathcal{K}:C\times V^* \rightarrow \mathfrak{X}^{**}$ as explained in \cite{HMR1998}, 
\[
\SCP{\mathcal{K}(gc, ag^{-1})}{\Ad^*_{g^{-1}}v} = \SCP{\mathcal{K}(c, a)}{v}
\,,\quad  \hbox{for all}\quad g \in G\,,
\]
for a manifold $C$ on which $G$ acts from the left. For fluid dynamics, $C$ is the space of loops the fluid domain $\mathcal{D}$ and the map $\mathcal{K}$ is the circulation around the loop. More specifically, for all $\alpha \in \Lambda^1$,
\begin{align}
    \SCP{\mathcal{K}(c, a)}{\alpha} := \oint_{c} \alpha,
\end{align}
    \begin{theorem}[SALT Kelvin-Noether theorem] \label{SKN theorem}
	Given solutions $m(t), a(t)$ satisfying the SALT LP equations \eqref{eq:SLP eq SALT} and fixed $c_0 \in C$, the associated Kelvin-Noether quantity $\SCP{\mathcal{K}(g(t)c_0, a(t))}{m(t)}$ satisfies the following stochastic Kelvin-Noether relation.
	\begin{align}
	\rmd \SCP{\mathcal{K}(g(t)c_0, a(t))}{m(t)} = \SCP{\mathcal{K}(g(t)c_0, a(t))}{\left(- \frac{\delta h}{\delta a}\,dt - \sum_i \frac{\delta h_i}{\delta a}\circ dW_t^i \right)\diamond a}
	\end{align}
	where we identify $\rmd g\,g^{-1} =: \rmd x_t$. 
\end{theorem}
%
\begin{remark}
    The proof of theorem \ref{SKN theorem} is in appendix \ref{app: KIW}. The fluid mechanics counterpart of the Kelvin-Noether theorem is expressed as
	\begin{align*}
	\rmd \oint_{c_t} \frac{m}{D} = \oint_{c_t} \frac{1}{D}\left(- \frac{\delta h}{\delta a}\,dt - \sum_i \frac{\delta h_i}{\delta a}\circ dW_t^i \right)\diamond a\,, 
	\end{align*} 
	where the material loop $c_t=g(t)c_0$ moves with stochastic velocity $\rmd g\, g^{-1}=\rmd x_t$ in equation \eqref{LagPath-SALT} and the quantity $D$ is the mass density of the fluid which is also advected as $D(t)=g_{t\,*}D_0$. That is, the mass density $D$ satisfies the stochastic continuity equation $\rmd D + \mathcal{L}_{\rmd x_t}D=0$.
\end{remark}

\begin{remark}[SALT Hamiltonians]
	In \cite{Holm2015}, the SEP equations are derived from a stochastic Clebsch variational principle where the advection of phase space Lagrangian variables are through a stochastic vector field $\rmd x_t = u\,dt + \sum_i \xi_i(x)\circ dW_t^i$. Compared to the stochastic vector field defined via $\rmd g\,g^{-1}$ in \eqref{eq:EP eq parts}, they coincide with those in \cite{Holm2015} when the noise Hamiltonians $h_i$ are linear in $m$, i.e. $h_i(m,a) = \SCP{\xi_i(x)}{m}$. The SEP equations then becomes
	\begin{align*}
	\rmd \frac{\delta \ell}{\delta u} = -\, \ad^*_{\rmd x_t}\frac{\delta \ell}{\delta u} + \frac{\delta \ell}{\delta a} \diamond a \,dt \,, \quad 
	\rmd a = -\mathsterling_{\rmd x_t} a\,, \quad \rmd x_t = u\,dt + \sum_i \xi_i(x)\circ dW_t^i\,.
	\end{align*}
	For data assimilation purposes, the choice $h_i(m,a) = \sum_i\langle m,\xi_i(x) \rangle$ was made in \cite{CCHOS18,CCHOS18a}.
\end{remark}
    
\end{framed}



==> scraps.tex <==
SCRAPS: 

\todo[inline]{DH: I'd say that $\rmd$ should be absent from \fbox{$\rmd$ b} in the previous equation \eqref{LDPaction w a}. \\
	Why is the $\rmd$ there? If it were to stay, we also would need a few more $dt$'s here to spell out what is being integrated.\\
	Personally, I would prefer the action integral in the form of the following equation.
	\begin{align}
	0=\delta S = \delta \int^b_a \ell(u,a) + \SCP{m}{ \dot{g}\, g^{-1} - u} + \SCP{ b}{a_0g^{-1} - a}\,dt - \int_a^b \sum_i\SCP{ad^*_u f^m_i}{\delta g\,g^{-1}}\circ dW^i_t.
	\label{LDPaction w a1}
	\end{align}
	This action integral in \eqref{LDPaction w a1} splits nicely into drift plus Stratonovich noise, without any need for $\rmd g$ and $ b$. \\
	RH: Yes both variational principle will give the same answer, the current one with $\rmd g\,g^{-1}$ and $ b$ makes it clear these are stochastic differential without specifying they have no dW parts. It also makes the Kelvin theorem easy to prove since we will take $\rmd$ of $g$.}


\todo[inline]{DH: I'd be more comfortable if the noises in the loop and in the integrand were different. However, that does not seem to be in the cards. }

\todo[inline]{We are thinking along the same lines, Ruiao.}

\section{Relation to the location uncertainty (LU) model}

Another stochastic fluid model which conserves kinetic energy known as location uncertainty (LU) was introduced by Mikulevicius and Rozovskii \cite{MikRoz2004} and Flandoli \cite{Flandoli2011} in their studies of well-posedness of stochastic partial differential equations and by M\'emin \cite{Memin2014} for more applied purposes. The LU framework has recently been successfully applied in quantifying uncertainty for two-dimensional geophysical fluid models by Resseguier et al. \cite{Resseguier2017}. For brief discussions of the comparison of LU with SALT, see \cite{Bauer-etal2020,RPFK2020}. 

\todo[inline]{DH: I think these three sentences and the eight references might be enough of an introduction to LU. Do you agree, Ruiao? 

I guess you are going amplify the steps in the equations below and put the final step in each example into vector calculus notation, right? }
Start with \eqref{LDP+SALT action} with arbitrary forcing $F^m_i$ only in $m$, 
	\begin{align}
	\begin{split}
	0 = \delta S &= \delta \int_{t_1}^{t_2} \SCP{m}{u} + \SCP{a}{b} - h(m,a) \,dt - \sum_i h_i(m,a)\circ dW^i_t - \int_{t_1}^{t_2}\SCP{F^m_i}{\eta} \circ dW^i_t\,.
	\end{split}
\end{align}
The resulting SFLP equations are
\begin{align}
\begin{split}
    &\rmd m + \ad^*_u m\,dt + b\diamond a\,dt +  \ad^*_{\xi_i} m\circ dW^i_t + F^m_i\circ dW^i_t = 0\,, \\
    & u = \frac{\delta h}{\delta m},\quad b =\frac{\delta h}{\delta a}, \quad \rmd a + \mathcal{L}_u a\,dt + \mathcal{L}_{\xi_i} a\circ dW_t^i = 0\,,
\end{split} 
\end{align}
where $\xi_i = \frac{\delta h_i}{\delta m}$. Compute the stochastic time derivative of energy to have
\begin{align*}
    \rmd h &= \SCP{\rmd m}{u} + \SCP{\rmd a}{\frac{\delta h}{\delta a}} = -\SCP{\ad^*_{\xi_i}m + F^m_i}{u}\circ dW^i_t 
\end{align*}
Defining $v = \left(\frac{1}{D}m\right)^\sharp$ where $D = \rho\, dV$ is the density and assuming $\xi_i$ are divergence free, $\rmd h$ can be written in terms of the $L^2(\mathfrak{X})$ inner product $\qp{\cdot}{\cdot}_{L^2(\mathfrak{X})}$ as
\begin{align}
    \rmd h = -\qp{\ad^\dagger_{\xi_i}v + \frac{1}{\rho}f_i}{u}_{L^2(\mathfrak{X})}\circ dW^i_t \label{SALT + SFLT erg time derivative}
\end{align}
where $f_i = \left(\frac{1}{dV}F^m_i\right)^\sharp$. 
\paragraph{3D Euler}
Assume for simplicity that $h = \int_\mathcal{D}|\bu|^2 dV$. Then density $D = dV$ and $v = u$. This simplifies \eqref{SALT + SFLT erg time derivative} to
\begin{align}
    \rmd h = -\qp{\ad^\dagger_{\xi_i}u + f_i}{u}_{L^2(\mathfrak{X})}\circ dW^i_t = -\qp{\ad_{\xi_i}u + f_i}{u}_{L^2(\mathfrak{X})}\circ dW^i_t
\end{align}
which vanishes when $f_i = -\ad_{\xi_i}u$. Thus $F^m_i = -\left(\ad_{\xi_i}u\right)^\flat dV$
\paragraph{RSW}
Now let $h$ be the RSW Hamiltonian \eqref{RSW Hamiltonian} where we let $\rho = \eta$ and $v = \epsilon\,u + r$ where $r$ is the vector field corresponding to constant vector $\bR$. Then \eqref{SALT + SFLT erg time derivative} simplifies to
\begin{align}
    \rmd h = -\qp{\ad^\dagger_{\xi_i}(\epsilon\,u+ r) + \frac{1}{\rho}f_i}{u}_{L^2(\mathfrak{X})}\circ dW^i_t = -\qp{\ad_{\xi_i}\epsilon u + \ad^\dagger_{\xi_i}r + \frac{1}{\rho}f_i}{u}_{L^2(\mathfrak{X})}\circ dW^i_t
\end{align}
which vanishes when $\frac{1}{\rho}f_i = -\ad_{\xi_i}\epsilon u - \ad^\dagger_{\xi_i}r $. Thus $F^m_i = -\left(\rho\,\ad_{\xi_i}\epsilon u + \rho\,\ad^\dagger_{\xi_i}r\right)^\flat dV$.

\begin{lemma}
    The term $\delta ((\rmd g, \rmd v)(g, v)^{-1}) = \delta (\rmd g\, g^{-1}, \rmd v \, g^{-1})$ can be written as
    \begin{align}
        \delta ((\rmd g,\rmd v)(g,v)^{-1}) = \rmd ((\delta g, \delta v)(g,v)^{-1}) - \ad_{(\rmd g, \rmd v)(g,v)^{-1}}(\delta g, \delta v)(g,v)^{-1},
    \end{align} 
    where the term $\delta (g,v) \in \mathfrak{s}$ is taken to be arbitrary and the adjoint operation on the semidirect product Lie algebra $\mathfrak{s} = \mathfrak{X}\circledS V$ is defined in Appendix \ref{app: semidirect ad^*}
    \end{lemma}
\begin{proof}
    Via direct calculation to have,
    \begin{align*}
        &\delta (\rmd g\, g^{-1}, \rmd v \, g^{-1}) = (\delta \rmd g\,g^{-1} - \rmd g\,g^{-1}\delta g\,g^{-1}, \delta \rmd v\,g^{-1} + \rmd v\,g^{-1}\delta g\,g^{-1})\\
        &\rmd ((\delta g, \delta v)(g,v)^{-1}) = \rmd (\delta g\,g^{-1}, \delta v\,g^{-1}) = (\rmd \delta g\,g^{-1} - \delta g\,g^{-1}\rmd g\,g^{-1}, \rmd \delta v\,g^{-1} + \delta v\,g^{-1}\rmd g\,g^{-1}).
    \end{align*}
    Subtracting the previously calculated tangent vectors and noting the cross derivative terms cancel to have
    \begin{align}
    \begin{split}
        \delta ((\rmd g, \rmd v)(g, v)^{-1}) - \rmd ((\delta g, \delta v)(g,v)^{-1}) &= (-\rmd g\,g^{-1}\delta g \,g^{-1} + \delta g\,g^{-1}\rmd g \,g^{-1}, -\rmd v\,g^{-1}\delta g\,g^{-1} + \delta v\,g^{-1}\rmd g\,g^{-1})\\
        &=([\rmd g\,g^{-1}, \delta g\,g^{-1}], -\rmd v\,g^{-1}\delta g\,g^{-1} + \delta v\,g^{-1}\rmd g\,g^{-1}) \\
        &= - \ad_{(\rmd g, \rmd v)(g,v)^{-1}}(\delta g, \delta v)(g,v)^{-1} 
    \end{split}
    \end{align}
\end{proof}
The variations thus becomes
\begin{align*}
\begin{split}
    0 = &\int_{t_2}^{t_1} \SCP{\delta(m,a)}{(\rmd g, \rmd v)(g,v)^{-1}} - \SCP{\delta(m,a)}{(\frac{\delta h}{\delta m}, \frac{\delta h}{\delta a})\,dt } +\SCP{(m,a)}{\delta((\rmd g,\rmd v)(g,v)^{-1})} \\
    &\qquad - \sum_i\SCP{\ad^*_{(\frac{\delta h}{\delta m}, \frac{\delta h}{\delta a})}(f^m_i, f^a_i)}{(\delta g, \delta v)(g,v)^{-1}} \circ dW^i_t \\
    = &\int_{t_2}^{t_1} \SCP{\delta(m,a)}{(\rmd g, \rmd v)(g,v)^{-1}} - \SCP{\delta(m,a)}{(\frac{\delta h}{\delta m}, \frac{\delta h}{\delta a})\,dt } - \sum_i \SCP{\ad^*_{(\frac{\delta h}{\delta m}, \frac{\delta h}{\delta a})}(f^m_i, f^a_i)}{(\delta g, \delta v)(g,v)^{-1}} \circ dW^i_t \\
    & \qquad +\SCP{(m,a)}{\rmd ((\delta g,\delta v)(g,v)^{-1}) - \ad_{(\rmd g, \rmd v)(g,v)^{-1}}(\delta g, \delta v)(g,v)^{-1}}  
\end{split} 
\end{align*}
This one yields stationary conditions
\begin{align}
(\rmd g, \rmd v)(g,v)^{-1} = \left(\frac{\delta h}{\delta m}, \frac{\delta h}{\delta a}\right)\,dt, \quad \rmd (m,a) + \ad^*_{(\rmd g, \rmd v)(g,v)^{-1}}(m, a) + \sum_i \ad^*_{(\frac{\delta h}{\delta m}, \frac{\delta h}{\delta a})}(f^m_i, f^a_i)\circ dW^i_t =0,
\end{align}
which assembles to the explicit semidirect product SFLP equation \eqref{ExplicitSDPergEqns}.
